$\phi$-Lagrangian, a new scalar mediator for light-by-light scattering process

The $\phi$ scalar boson is a new mediator proposed to describe the direct light-by-light scattering observed recently in ultra-peripheral collisions (UPCs) with ATLAS detector where two photons interact directly to gives two photons in the final state. The proposed lagrangian present a description to the forbidden process. The description presented in this paper consist the interaction terms, the coupling to the Higgs boson to generate the mass for this new resonance and the simulation using proton proton in order to observe this process in other nominal LHC collisions, since the process is observed in heavy-ions collisions.

==> sec5.tex <==
\section{Search for $\phi$}
As I mention before in this section I will describe a new strategy to search for this mediator, the idea is basically search for signature of di-Z bosons scattering bellow the Higgs peak. The evidence of di-Z bosons scattering with the low cross section is a very good argument of the existence  new physics beyond SM (BSM) at low mass.\\

\subsection{R-ratio}
R-ratio is the ratio between cross section of di-Z and di-$\gamma$ scattering computed using (\ref{eq:eq1}):
\begin{equation}
	\mathcal{R} = \frac{\sigma(zz\rightarrow zz)}{\sigma(\gamma\gamma\rightarrow\gamma\gamma)}
\end{equation}
\begin{equation}
	\mathcal{R} = \frac{\tan^8_{\theta_w}}{36}(8+B(s,m_z))^2
\end{equation}
B is a function of energy s and Z-boson mass. \\

\begin{equation}
	B(s,m_z) = (\frac{s-2m^2_z}{m^2_z})^2
\end{equation}

R will be a discriminate variable to associate the di-Z bosons signature to the new $\phi$ exchanging.
